Geo-Spotting: Mining Online Location-based Services for Optimal Retail Store Placement

The problem of identifying the optimal location for a new retail store has been the focus of past research, especially in the field of land economy, due to its importance in the success of a business. Traditional approaches to the problem have factored in demographics, revenue and aggregated human flow statistics from nearby or remote areas. However, the acquisition of relevant data is usually expensive. With the growth of location-based social networks, fine grained data describing user mobility and popularity of places has recently become attainable. In this paper we study the predictive power of various machine learning features on the popularity of retail stores in the city through the use of a dataset collected from Foursquare in New York. The features we mine are based on two general signals: geographic, where features are formulated according to the types and density of nearby places, and user mobility, which includes transitions between venues or the incoming flow of mobile users from distant areas. Our evaluation suggests that the best performing features are common across the three different commercial chains considered in the analysis, although variations may exist too, as explained by heterogeneities in the way retail facilities attract users. We also show that performance improves significantly when combining multiple features in supervised learning algorithms, suggesting that the retail success of a business may depend on multiple factors.

==> evaluation.tex <==
As discussed, a principal aim of this paper is to identify the 
most important information signals that can be mined from location-based services,
in order to forecast the number of check-ins a retail store may attract when placed at
an area. To this end, we evaluate the performance of 
individual prediction features introduced in the pervious section. 
We first describe the methodology and the metrics 
we employ; then we compare the performance of each individual feature
across these metrics. Finally, we study the effect on prediction performance when altering
the radius $r$, which defines the area of investigation surrounding the retail facility.

\subsection*{Methodology and Metrics}
Given a specific retailer brand like the three we are considering in this paper,
we analyse a set of prediction areas $L$ to open a new store. 
For each feature and area $l \in L$ we compute a numeric value $\chi_l$ and rank the 
locations based on this.
As a result we obtain a ranked list of locations $R = (l_1, l_2, ..., l_{|L|})$
and denote with $rank(l_i)$ position of location $l_i$ in $R$. 
We also compute the ranked list $\overline{R}$ of locations based on the actual popularity (number of check-ins)
of the stores in those locations and denote with 
$\overline{rank}(l)$ the position of location $l$ in $\overline{R}$. 
Given the two lists ranking locations in terms of predicted and ground truth values, 
we can formally define the metrics we use to assess
the quality of predictions achieved by the different features.
% we compare the predicted ranking of locations $R$ with the ranking 
% based on actual popularity $\overline{R}$ using several performance metrics. 
\newline
\textbf{Normalized Discounted Cumulative Gain for top-K locations:}
Firstly, we aim to measure the extent to which the top-k locations in the list of actual popularity 
$\overline{R}$ are highly ranked in the predicted list $R$. To this end, we adopt 
the $NDCG@k$ (Normalized Discounted Cumulative Gain) metric frequently used in the 
performance evaluation of information retrieval systems \cite{jarvelin2002cumulated}. The metric assesses
the cumulative gain achieved by placing the most relevant instances in the top-k 
of the prediction list as formally defined by the Discounted Cumulative Gain measure:
\begin{equation}
DCG_k = \sum_{i = 1}^{k}{\frac{2^{rel(l_i)}-1}{\log_2{(i+1)}}}
\end{equation}
where $rel(l_i)$ is the relevance of an instance at position $i$ in the predicted ranking $R$.  
The result is then normalized by the $DCG$ of the ideal prediction ($iDCG$), i.e.,  
when the instances are sorted by the relevance with the most relevant in the first position. 
The resulting scores, thus, lie in the range from $0 < NDCG@k \leq 1$. We
define the relevance of an instance as its relative position in the 
actual ranking $\overline{R}$, i.e., $rel(l_i) = \frac{|L| - \overline{rank}(l_i) + 1}{|L|}$.
The $rel(l_i)$\ta{Before you defined it differently. Please clarify.} score is equal to $1$ when the area is ranked first in terms of check-ins 
and it linearly decreases to $0$ as the rank goes down the list. As a baseline for comparison 
we use the expected value of $NDCG@k$ for a random ranker, i.e., the result achieved by randomly 
permuting the instances. 
\newline
\textbf{Assessing the Best Prediction:}
Consindering now the application scenario where the best geographic area has to be elected, for instance 
by a geo-analytics team, we would like to test the quality of the top-ranked location usually 
attained by the different ranking strategies. 
% We measure the relevance of the best prediction, \emph{RelTop}, that is the relative 
% position of the top predicted place $l_1$ in the actual popularity ranking $\overline{R}$, i.e., $RelTop = rel(l_1)$. 
% The expected value of $RelTop$ score for a random ranker is equal to $0.5$, i.e., when the top predicted location lies 
% in the middle of the actual popularity list. 
We then measure the probability of the best predicted location 
to be amongst the \emph{Top X}$\%$ most popular areas. 
We measure the accuracy of the best prediction as the successful prediction of the best 
location in the \emph{Top X}$\%$ of the acctual popularity list $\overline{R}$, i.e.,
\ta{That is unclear: best, successful, top? can you clarify please?} 
for a given $X\%$ of the most popular areas, prediction is successful if $(1 - RelTop) \times 100\% \leq X\%$. 
\ta{Rename reltop or redefine to something else as its not relevant anymore}.
Average accuracy, which we denote as \emph{Accuracy@X$\%$}, is the fraction of successful experiments over 
the total number of prediction tasks and, thus, corresponds to the probability of having the \emph{Top X}$\%$
area on the first place in the predicted ranking $R$. Here, we use the percentage of the list $X\%$, 
rather than the absolute top-k values, since we would like to compare all three chains using the same baseline for the 
random ranker, i.e., $Accuracy@X\% = X\%$, given that the number of places per chain may vary.

\newline
\textbf{Geographic Cross Validation:}
We use a random sub-sampling method \cite{maimon2010} to 
select subsets of geographic areas for validation.
In each experiment we randomly sample 33\% of the total areas 
associated with the stores of the brand we analyse, obtaining $L$ candidate areas for prediction.
The rest of the areas are subsequently used to form our training set where features (or supervised learning
algorithms as we see in Section~\ref{sec:supervised}) will be trained.
We assume that the stores in the test 
set areas $L$ do not yet exist and our goal is to forecast 
the popularity ranking of the stores, if they were
to be opened there. 
All scores are measured by averaging $100$ times the cross validation 
method over geographic areas described above.
%  NDCG@$10$ and RelTop across all experiments, i.e., \emph{Average
% NDCG@$10$} and \emph{Average RelTop}.

\begin{table}[htbp]
\begin{center}
	\begin{tabular}{|c|c|c|c|}
		\hline
		\textbf{Feature} & \textbf{Starbucks} & \textbf{Dun.Don.} & \textbf{McDon.} \\ \hline
		\multicolumn{4}{|c|}{\textbf{Geographic Features}} \\ \hline
		Density 			 			& 0.60 & 0.79 & 0.73 \\ \hline
		Entropy 			 			& 0.65 & 0.60 & 0.69 \\ \hline
		Competitiveness 		& \textbf{0.70} & 0.68 & \textbf{0.78} \\ \hline
		Jensen Quality 			& 0.54 & \textbf{0.81} & 0.72 \\ \hline
		\multicolumn{4}{|c|}{\textbf{Mobility Features}} \\ \hline
		Area Popularity 		& 0.54 & 0.77 & 0.78 \\ \hline
		Transition Density 	& 0.62 & 0.79 & 0.78 \\ \hline
		Incoming Flow   		& 0.60 & 0.75 & \textbf{0.79} \\ \hline
		Transition Quality 	& \textbf{0.66} & \textbf{0.81} & 0.73 \\ \hline
		\multicolumn{4}{|c|}{\textbf{Random Baseline}} \\ \hline
		                    & 0.48 & 0.51 & 0.53 \\ \hline
	\end{tabular} 
\end{center}
	\caption{The Average NDCG@10 results of the individual features predictions 
	for each of the three chains.}
	\label{table:individual_ndcg}
\end{table}


\subsection*{Individual Feature Performance}
		\textbf{Top-K location ranking:}
		The results based on the NDCG@10 metric for all features across different chains are presented in Table~\ref{table:individual_ndcg}.
		All features perform considerably better than the random scenario, i.e., when the ranking is achieved by randomly
		permuting the instances. The best performing feature in the category of geographic features is \texttt{Competitiveness} for 
		McDonalds and Starbucks, and \texttt{Jensen's Quality} for Dunkin' Donuts.  
		The deviation of the Dunkin' Donuts case can be possibly explained by the fact that these restaurants 
		benefit more from the co-location with other places, as measured by \texttt{Jensens' Quality}, 
		than from being in an environment with less competition. This hypothesis is supported by the 
		fact that Dunkin' Donuts restaurants are often placed close to gas stations 
		(as we observed in Table~\ref{table:jensen}). \dk{rephrase this argument}
		Overall, the features that consider the types of 
		the surrounding places give better signal of the attractiveness of the location than 
		general density and popularity measures highlighting perhaps how semantics is an important information source
		in location based services. 

	  	With respect to the class of mobility features we have mined,
		the best performing characteristic in case of McDonald's is the \texttt{Incoming Flow}, 
		which measures user mobility towards from remote areas. For the other two cases (Starbucks and Dunkin' Donuts) top performer is 
		\texttt{Transition Quality}, which exploits the flow of users from nearby places. 
		In all cases the best performing features considerably outperform the naive 
		\texttt{Area Popularity} baseline. This finding 
		suggests that just knowing how busy an area is in terms of number of check-ins, may not be the best predictor 
		for placing a retail store as could be inferred intuitively. 
		As a general remark, we observe that some features, such \texttt{Competitiveness}, \texttt{Density of 
		Transitions} and \texttt{Incoming Flow} are good indicators of the place quality across 
		all considered chains, while others, such as \texttt{Transition Quality} or \texttt{Entropy}, 
		depend on the specific chain.
	% 			\begin{figure}[ht]
	% 	\centering
	% 	\includegraphics[width=1.0\columnwidth]{./figures/features-performance}
	% 	\caption{The Average RelTop of the individual features predictions 
	% for each of the three chains. The features are grouped in two classes: Geographic Features,
	% which are based on characteristics of the nearby places, and Mobility Features, 
	% which take into account human mobility flows in the area}
	% 	\label{fig:features_pr}
	% 	\end{figure}
		\begin{figure*}[htbp]
			\centering
			\includegraphics[width=0.66\columnwidth]{./figures/topx_starbucks}
			\includegraphics[width=0.66\columnwidth]{./figures/topx_dunkindonuts}
			\includegraphics[width=0.66\columnwidth]{./figures/topx_mcdonalds}
			\caption{The Accuracy@X\% results of the individual features predictions for Starbucks (left), Dunkin' Donuts (center) and McDonalds (right).}
			\label{fig:accuracy}
		\end{figure*}
		\newline
		\textbf{Best location prediction results:}
		% We now analyse the relevance of the top predicted location as assessed by the Average
		% RelTop metric. The corresponding results for all three chains are presented 
		% in Figure~\ref{fig:features_pr}. Overall, the result is in general agreement with the 
		% corresponding results for the top-k prediction, as assessed by the $NDCG@10$ metric. However, 
		% we also observe some deviations in the best performing indicators, the finding that suggests 
		% that two problems has to be analysed individually. Thus, in the geographic features category, \texttt{Competitiveness} is the best 
		% indicator of the optimal location in all three chains, outperforming the \texttt{Jensen's Quality} 
		% as the best predictor for Dunkin' Donuts according to the $NDCG@10$-based assessment. Similarly, the \texttt{Transitional Quality} 
		% slightly outperforms the \texttt{Incoming Flow} indicator for the optimal Dunkin' Donuts location predictor
		% in comparison with the corresponding results for the top-k prediction. 	
		To assess the probability of the most highly ranked location to be amongst the \emph{Top X}$\%$ most popular areas
		we measure the $Accuracy@X\%$ for different portions of top lists $X$. We plot the results in Figure~\ref{fig:accuracy} along with the 
		corresponding expected value for the case when the best location is selected randomly among all candidates 
		(black solid line in the plot). All features except \texttt{Entropy} perform significantly better than the random scenario for 
		list portions larger than 10\% in the cases of Dunkin' Donuts and McDonald's, whereas performance drops to 25\% in the case of Starbucks. 
		Further, accuracy approximates a $90\%$ score when considering the Top $30\%$ of the list
		for the optimal Dunkin' Donuts placement and the level of $83\%$ for the \texttt{Competitiveness}-based prediction 
		in the same setting. The situation is slightly different for the accuracy of prediction 
		in the Top $10\%$ of the candidate list. For example, the peak performing feature of $Accuracy@30\%$ prediction - 
		the \texttt{Density} feature - is not effective when we consider smaller portions of top lists $X$. Instead, when considering 
		prediction performance of the \texttt{Competitiveness} feature one can spot the Top $10\%$ places for a Dunkin' Donuts 
		restaurant with relatively high accuracy of $58$\%. That signifies that lack of competition in the area may 
		be a promising signal to exploit when opening a new retail store. \dk{shorten this section slightly}
	%	Instead, with Competitiveness-based prediction 
	%	one can spot the Top $10\%$ places for a Dunkin' Donuts restaurant with relatively high accuracy of 67\%. 
		\newline
		\textbf{Controlling for area radius r:} Finally, we study the influence of the parameter $r$ which corresponds to the radius of the area around 
		the geographic spot we examine. We plot in Figure~\ref{fig:radius} the $NDCG@10$ results for individual features as a function of 
		the radius measured for the chain with the biggest number of stores, i.e., Starbucks. 
		The maximum performance across the majority of the features is achieved for $r = 200m$. 
		This finding can be explained as a result of a trade-off between being geographically specific 
		in the definition of the area for feature mining, but also able to incorporate as much information
		as possible about the surroundings. If the radius is too small, it does not cover all of places nearby 
		that may provide useful information. On the other hand,
		if the radius is too broad, then some places are too distant to be considered influential 
		to the geographic spot in question. The radius size of $200$ meters is also in agreement 
		with what the urban planning community considers as the optimal neighborhood size \cite{mehaffy2010}.
 		% for a potential fast-food or coffee-shop client are also put in the equations, thus, 
		% creating a noise in the prediction signals. 
		% TODO: reference some previous findings as Cecilia sugggested
		\newline
		\textbf{Take away message:}
		As the main result of our analysis we conclude that the information on types and 
		surrounding objects as well as on human mobility patterns in the surrounding area 
		can be effectively explored to assess the retailer quality of the location and 
		spot the areas where a new store will attract maximum number of check-ins. 
		Particularly, we show that the analysis of the transition-based metrics, 
		such as the \texttt{Incoming Flow} of users towards the area under analysis,
		the \texttt{Density of Transitions} inside the area and the estimation of the 
		potential flows of users from the nearby places as assessed by 
		the \texttt{Transitional Quality}, yields the best performance results for the 
		optimal retail location evaluation. Finally, we show that the radius 
		of $200m$ is the optimal value for the surrounding area selection.		 
		
\section{Supervised Learning Approach}
\label{sec:supervised}
	In this section we combine our features in a supervised 
	learning framework. Our aim is to exploit the union of individual 
	features in order to improve predictions, assuming that the popularity 
	of places in Location-based Social Networks can by predicted by considering 
	a composition of factors. We consider several different supervised models to learn how feature
	vectors $\mathbf{x}$ can be associated with the check-in scores $y$ of the areas under prediction: Linear 
	Regression with regularization, Support Vector Regression and M5 decision trees \cite{quinlan1992}, \cite{hearst1998}. 
	We have used the corresponding implementations that are publicly available through the 
	WEKA machine learning framework \cite{witten2011}. By training the supervised learning algorithms to 
	obtain regression scores and subsequently rank the candidate geographic areas, we are essentially reducing 
	the regression problem to a ranking one. 
	
	\dk{cut some the algorithm description, too long}
	
		\begin{figure}[ht]
		\centering
		\includegraphics[width=1.0\columnwidth]{./figures/features_from_radius}
		\caption{The Average NDCG@10 values of the individual features predictions measured for different values of the area radius $r$.}
		\label{fig:radius}
		\end{figure}\dk{The old figure - has to be updated}
		
	Additionally, we consider a pair-wise learning-to-rank approach, RankNet \cite{burges2005learning},
	that learns to classify ordering relation between a pair of venues basing on their features, i.e., given a pair of
  venues $A$ and $B$, characterized by features $\mathbf{x^A}$ 
  and $\mathbf{x^B}$, identify if venue $A$ has to be ranked 
  higher than $B$. The models assume a ranking function $H(\mathbf{x}) : \Re^{|\mathbf{x}|} \rightarrow \Re$ such 
  that the rank order of a set of test samples is specified 
  by the real values that $H$ takes, specifically, 
  $H(\mathbf{x^A}) > H(\mathbf{x^B})$ is taken to mean that 
  model asserts that $A \succ B$. As a ground truth in this model 
  we explore a linear ranking $\overline{R}$ of the training and testing venues 
  according to their number of check-ins. The testing and evaluation of the supervised 
  algorithms is conducted using the exact methodology
	we have used for the evaluation of individual features, and all features have been normalized 
	before training.
	
	The regularized linear regression model assumes that 
	the output score $y$ is a linear combination of the input features $\mathbf{x}$ with the weights
	being calculated from the training data. The goal of the prediction 
	algorithm is to minimize the error between actual and predicted outputs:
	\begin{align}
		\underset{\textbf{w}} \min \Vert\mathbf{x}^{\mathsf{T}} \mathbf{w} - y \Vert^{2} + \gamma \Vert\mathbf{w}\Vert^{2}
		% \min_{w}||x^Tw - y||^2
	\end{align}
	where $\gamma$ is the regularization parameter set here equal to $10^{-8}$.

	Support Vector Regression belongs in the family of generalized linear regressors
	and also assume a linear model to 
	minimize prediction error, however, in this case all deviations up to a 
	specified level $\epsilon$ are discarded during training. The algorithm 
	tends to reduce the risk of over-fitting by trying to maximize 
	the flatness of the learned function while minimizing the error. For non-linear problems the algorithm
	applies a kernel function to transform the features space to a more linear one. 
	
	The M5 model tree is an approach based on continuous decision tree
	learning \cite{quinlan1992}.  The principal advantage offered by M5 trees is their
	ability to produce continuous numerical outputs, rather than binary categories
	as usually inferred by decision trees. That is desirable in the present context
	as we want to rank geographic areas according real valued scores. This is achieved
	by creating a decision tree that splits learning instances according to
	their features: on each leaf a subset of the features contained in $\mathbf{x}$
	is used in a linear regression model to output a numeric score.
	Typically nodes in decision trees employ a threshold on a certain feature to
	split the training set $T$. Unlike other decision trees where the information gain
	criterion is used to choose the attribute to split on, M5 model trees split on
	the attribute which maximizes the expected error reduction.  Formally, the
	standard deviation reduction (SDR) is defined as
	% 
	% In the M5 decision trees prediction model contains a set of different linear 
	% function one of each is applied depending on the output of associated decision tree.  
	% The decision tree is constructed by splitting the learning instances according 
	% to their features. Then on each leaf a subset of the features contained in $x$ is used in a linear 
	% regression model to output a numeric score. Typically nodes in decision employ a threshold on a certain
	% feature to split the training set. These decision attributes are selected to maximize the expected 
	% reduction error.
	\begin{equation*} SDR =  sd(T)
	  - \displaystyle\sum \frac{|T_{i}|}{|T|} \times sd(T_{i}) 
	\end{equation*} where
	  $T$ is the set of training examples that reach the node and $T_{1}, T_{2} ...$
	  are the sets that result from splitting the node to the chosen attribute.

	In the RankNet algorithm the ranking function $H(x)$ is 
	modeled as a neural network. The output of the algorithm is mapped to the probability $P_{AB}$ that 
	venue $A$ is to be ranked higher than venue $B$ with a logistic function 
	$P_{AB} = \frac{e^{o_{AB}}}{1 + e^{o_{AB}}}$, where $o_{AB} = H(A) - H(B)$ is 
	a distance between the ranks of $A$ and $B$. The neural network is then trained 
	with a gradient algorithm to minimize the 
	loss function defined as pair-wise cross entropy between the target value
  $\overline{P}_{AB}$ and the modeled probability $P_{AB}$, i.e.,:  

	\begin{equation} 
    C_{AB} = H(\overline{P}_{ij},P_{ij}) = o_{ij} + log(1 + e^{o_{ij}})
  \end{equation} 


%	\begin{table*}[htbp]
%	\begin{center}
%		\begin{tabular}{|c|c|c|c|}
%			\hline
%			\textbf{Algorithm} & \textbf{Starbucks} & \textbf{Dunkin' Donuts} & \textbf{McDonald's}\\ \hline
%			\multicolumn{4}{|c|}{\textbf{Geographic Features}} \\ \hline
%			Linear Regression 				& 0.78 & 0.84 & 0.80 \\ \hline
%			M5 Decision Trees 				& 0.76 & 0.84 & 0.80 \\ \hline
%			Support Vector Regression & 0.78 & 0.88 & 0.84 \\ \hline
%			\multicolumn{4}{|c|}{\textbf{All Features}} \\ \hline
%			Linear Regression 				& 0.90 & 0.88 & 0.90 \\ \hline
%			M5 Decision Trees 				& 0.89 & 0.88 & 0.91 \\ \hline
%			Support Vector Regression & 0.87 & 0.90 & 0.91 \\ \hline
%		\end{tabular} 
%	\end{center}
%		\caption{The best APR results of the supervised learning algorithms applied to combinations of features 
%		geographic features.}
%		\label{table:combination}
%	\end{table*}

	\begin{table}
	\begin{center}
		\begin{tabular}{|c|c|c|c|}
			\hline
			\textbf{Algorithm} & \textbf{Starbucks} & \textbf{Dun.Don.} & \textbf{McDon.}\\ \hline
			\multicolumn{4}{|c|}{\textbf{Geographic Features}} \\ \hline
			Lin. Regression 		& 0.73 & 0.80 & 0.78 \\ \hline
			M5 Dec. Trees 			& 0.72 & 0.80 & 0.78 \\ \hline
			SVR                 & 0.73 & 0.81 & 0.81 \\ \hline
			RankNet             & 0.72 & 0.81 & 0.79 \\ \hline
			\multicolumn{4}{|c|}{\textbf{All Features}} \\ \hline
			Lin. Regression 		& 0.76 & 0.82 & 0.82 \\ \hline
			M5 Dec. Trees 			& 0.77 & 0.82 & 0.82 \\ \hline
			SVR                 & 0.77 & 0.83 & 0.84 \\ \hline
			RankNet             & 0.77 & 0.81 & 0.83 \\ \hline
			\multicolumn{4}{|c|}{\textbf{Random Baseline}} \\ \hline
		                      & 0.48 & 0.51 & 0.53 \\ \hline
		\end{tabular} 
	\end{center}
		\caption{The best Average NDCG@10 results of the supervised learning algorithms applied to combinations of features 
		grouped into two classes: combinations of geographic features only and combinations of both mobility and 
		geographic features.}
		\label{table:combination}
	\end{table}
			
	\paragraph{Results}
	
			We now present the results of supervised learning using four different algorithms. 
			We measure performance of the algorithms trained separately on different combinations of 
			geographic features and then combining them with mobility features. This way we aim to assess the
			extent to which the fusion of the features yields better results 
			than the prediction based on individual features and secondly, to which extent adding mobility 
			features improves predictability based only on geographical information. 
			The supervised models based on the grouping of geographic features have a slight
			increase ($0.2$-$0.3$) of $NDCG@10$ performance in comparison to individual feature prediction 
			in two of three cases, i.e., McDonalds and Starbucks. Instead, adding mobility features to the supervised model 
			considerably improves the prediction results (Table~\ref{table:combination}) across all chains. 
			Thus, for example, the best result of supervised 
			learning for Starbucks, an $NDCG@10$ score of $0.77$, 
			improves the performance of \texttt{Transition Quality}, our best single feature prediction, 
			by $0.07$. In the Dunkin' Donuts and McDonald's cases the best $NDCG@10$ in 
			supervised learning reaches the mark of $0.83$ and $0.84$ in comparison to the best single feature performance that achieves 
			$0.81$ and $0.79$ correspondingly. 
			
					\begin{figure}[ht]
		\centering
		\includegraphics[width=1.0\columnwidth]{./figures/algorithms-performance}
		\caption{The Average RelTop of the individual features predictions 
	for each of the three chains. The features are grouped in two classes: Geographic Features,
	which are based on characteristics of the nearby places, and Mobility Features, 
	which take into account human mobility flows in the area}
		\label{fig:algorithms_pr}
		\end{figure}
	
	
%			We now present the results of supervised learning using three different algorithms. 
%			We measure performance of the algorithms trained separately on different combinations of 
%			\emph{Geographic} features and then combining them with \emph{Mobility} features. This way we aim to assess the
%			extent to which extent the fusion of the features yields better results 
%			than the prediction based on individual features and secondly, to which extent adding mobility 
%			features improves predictability based only on geographical information. 
%			The supervised models based on the grouping of geographic features have a slight
%			increase of $1-2\%$ in comparison to individual feature performance in two of three cases, i.e., Starbucks and Dunkin' Donuts.
%			Instead, adding mobility features to the supervised model 
%			considerably improves the prediction results (Figure~\ref{fig:algorithms_pr}) across all chains. Thus, for example, the best result of supervised 
%			learning for Starbucks, an APR score $(90\%)$, improves the performance of \emph{Transition Quality}, our best single feature prediction, 
%			by $14\%$. In the Dunkin' Donuts and McDonald's cases the best APR in 
%			supervised learning reaches the mark of 90\% and 91\% in comparison to the best single feature performance that achieves 87\% and 86\% correspondingly. 

			Across different combination of features we observe that the best prediction performance is achieved 
			when combing transition-based metrics, i.e., \texttt{Incoming Flow}, \texttt{Transition Density} and \texttt{Quality Transition}, 
			with geographic features assessing heterogeneity and competitiveness of the surrounding environment, i.e., 
			\texttt{Entropy}, \texttt{Jensen's Quality} and \texttt{Competitiveness}. Thus, for McDonalds the top performing 
			combination is \texttt{Transition Density}, \texttt{Incoming Flow}, \texttt{Competition} and \texttt{Entropy}. 
			The result of the Dunkin' Donuts case is similar, however, the performance is even more improved 
			if considering also the \texttt{Density} of the surrounding places. Instead, for Starbucks 
			the best combination of features is achieved when the \texttt{Transition Density} is substituted
			with the \texttt{Transition Quality}. The result is well aligned with the fact that for Starbucks performance of the individual 
			feature prediction based on the \texttt{Transition Density} feature is significantly lower than 
			performance of the \texttt{Transition Quality}-based prediction (see Table~\ref{table:combination}). 
			While comparing the performance of different supervised learning algorithms considering the NDCG@10 score, 
			we have not observed large variability across the three cases, but we note that the performance of the 
			Support Vector Regression have offered better results for all considered chains. 

%			Interestingly, we have observed that the best performing combination of features across different chains are slightly different. 
%			Thus, for Starbucks, the combination of \emph{Jensen Quality}, \emph{Competitiveness} and \emph{Quality Transition} yields the 
%			highest NDCG@10. Instead, for McDonald's, the highest performance is achieved with a similar combination of the first two ingredients
%			but substituting \emph{Quality Transition} with \emph{Transition Density}. The result is well aligned with the fact that 
%			for McDonald's performance of the individual feature prediction based on the \emph{Quality Transition} feature is significantly lower than 
%			performance of the \emph{Transition Density}-based prediction (see Table~\ref{table:combination}). 
%			While comparing the performance of different supervised learning algorithms considering the RelTop score, 
%			we have not observed large variability across the three cases, but we note that the performance of the 
%			Support Vector Regression and M5 Model Trees have offered better results for the cases of Dunkin' Donuts 
%			and Mc Donald's, whereas the regularized linear regression has achieved best performance in the case
%			of Starbucks.\dk{rewrite this section}

		\begin{figure}[ht]
		\centering
		\includegraphics[width=0.90\columnwidth]{./figures/topx_all}
		\caption{The Accuracy@X\% results of the best performing combination of features for the three store chain.}
		\label{fig:combination}
		\end{figure}
		
			The improvement in performance when supervised learning is applied is more clearly indicated when 
			we consider the top one predicted location. Thus, for example, the best result of supervised 
			learning for Starbucks, an RelTop score $(98\%)$, improves the performance of \emph{Transition Quality}, 
			our best single feature prediction, by $22\%$ (see Figure~\ref{fig:algorithms_pr}). In the Dunkin' Donuts and McDonald's cases the best 
			RelTop in supervised learning reaches the mark of 94\% in comparison to the best single feature performance that 
			achieves 87\% and 86\% correspondingly. The top inferred geographic area for Starbucks, as shown in Figure~\ref{fig:combination}, 
			is positioned with an Accuracy of $65\%$ and $77\%$ amongst the \emph{Top 10\%} and the \emph{Top 15\%} most popular places respectively. 
			When considering the \emph{Top 20\%} most popular places, Accuracy goes over the mark of $80\%$ across all considered chains, reaching 
			a maximum of $83\%$ in the case of Dunkin' Donuts. These results significantly outperform the best individual features 
			predictions that are $58\%$ for Starbucks, $70\%$ and $78\%$ for McDonald's and Dunkin' Donuts respectively. 
			
			As expected, the combination of geographic and mobility features in a supervised learning algorithm 
			yields better results than the single feature based predictions. Moreover, when considering mobility features in 
			addition to the geographic features we have observed large improvements, highlighting that information about 
			the check-in movements of Foursquare users can add value in predicting a retail area of high quality. 
			Particularly, we show that the combination of the transition-based metrics, 
			i.e., \emph{Incoming Flow}, \emph{Transition Density} and \emph{Quality Transition}, 
			with the geographic features assessing heterogeneity and competitiveness of the surrounding environment, i.e., 
			\emph{Entropy}, \emph{Jensen's Quality} and \emph{Competitiveness}, yields the best prediction performance. Across 
			different prediction techinques we observed that the best performance is achieved for the predictions based 
			on the Support Vector Regression algorithm. 
			
			
			
